On the Efficient Implementation of High Accuracy Optimality of Profile Maximum Likelihood

We provide an efficient unified plug-in approach for estimating symmetric properties of distributions given $n$ independent samples. Our estimator is based on profile-maximum-likelihood (PML) and is sample optimal for estimating various symmetric properties when the estimation error $\epsilon \gg n^{-1/3}$. This result improves upon the previous best accuracy threshold of $\epsilon \gg n^{-1/4}$ achievable by polynomial time computable PML-based universal estimators [ACSS21, ACSS20]. Our estimator reaches a theoretical limit for universal symmetric property estimation as [Han21] shows that a broad class of universal estimators (containing many well known approaches including ours) cannot be sample optimal for every $1$-Lipschitz property when $\epsilon \ll n^{-1/3}$.

==> alg_iteration_i.tex <==
\section{Proof of \Cref{lem:iteri}}
Here we provide the analysis for each iteration of the for loop in \Cref{alg:main} and prove \Cref{lem:iteri}. 
\begin{proof}[Proof of \Cref{lem:iteri}]
We prove this lemma through induction. 
\paragraph{Base case i=0}
In this case $\mx^{(0)}=\mx$, $\my^{(0)}=\mx$, $\bR^{(0)}$ and $v^{(0)}$ is an empty vector. As $\mx \in \bZfrac$, we have that all the conditions of the lemma are immediately satisfied. We remark that conditions $(b)$, $(c)$ and $(a2)$ are empty for case $i=0$.

\paragraph{Inductive step $i$}
We assume that the lemma conditions hold for $i-1$ and prove for the case $i$. Therefore we are given that,
\newcommand{\myimt}{\my^{(i-2)}}
\newcommand{\vimo}{\textbf{v}^{(i-1)}}
\begin{itemize}
\item The matrix $\mximo \in \R_{\geq 0}^{\ell \times k}$ and satisfies the following inequalities:
        \begin{itemize}
            \item $\sum_{i' \in [\ell]}\mximo_{i'j} \in \Z_{\geq 0} \text{ for all } j \in [0,k]$.
            \item $\sum_{j \in [k]}\mximo_{i'j} \in \Z_{\geq 0} \text{ for all } i' \in [i-1]$.
        \end{itemize}
        \item The row vector $\vimo \in \R_{\geq 0}^{[0,k]}$ has integral row sum, that is,
        $\sum_{j \in [0,k]} \vimo_{j} \in \Z_{\geq 0}~.$
        \item The matrix $\myimo \in \bZimo$ and $\bg(\myimo) \geq \exp(-\log n) \bg(\myimt)$.
\end{itemize}
For iteration $i$, note that the matrix $\mximo$ and index $i$ satisfy the requirements of the routine $\pround$ and by \Cref{lem:partial-round} we get a matrix $\my \in \R_{\geq 0}^{\ell \times [0,k]}$ and a column index $j$  such that, $\|\my-\mximo\|_1\leq O(1)$ and,
\begin{align}
  & \bullet \sum_{i' \in [\ell], j'\in [0,k]} m_{j'} \log r_{i'} \my_{i'j'} \geq \sum_{i' \in [\ell], j'\in [0,k]} m_{j'} \log r_{i'} \mximo_{i'j'}  \bullet ~\sum_{i' \in [\ell]}\my_{i'j'}=\sum_{i' \in [\ell]}\mximo_{i'j'} \text{ for } j' \in [0,k] \label{eq:b2}\\
  &\bullet ~\sum_{j' \in [0,k]}\my_{i'j'} =\sum_{j' \in [0,k]}\mximo_{i'j'} \text{ for all } i' \in [\ell]
  ~~\bullet ~\my_{ij} \geq o \text{ and } \sum_{i'=1}^{i-1} \my_{i'j}+\my_{ij}-o \in \Z_{\geq 0}, \label{eq:c2}
\end{align}
where $o=\sum_{j' \in [0,k]}\mximo_{ij'} - \lfloor \sum_{j' \in [0,k]}\mximo_{ij'} \rfloor$. Furthermore, by \Cref{lem:lips}, $\sum_{i \in [\ell], j\in [0,k]} m_j \log r_i \my_{ij} \geq \sum_{i \in [\ell], j\in [0,k]} m_j \log r_i \mximo_{ij}$ and combined with $\|\my-\mximo\|_1\leq O(1)$ we get that,
\begin{equation}\label{eqy1}
    \bg(\my) \geq \exp(-O(\log n)) \bg(\mximo)~.
\end{equation}
Note that the matrix $\my$, row index $i$ and column index $j$ satisfy the requirements of the algorithm $\roundi$ and by \Cref{lem:roundi} we get that the matrix $\mxi$, $\vi$ and $\rnew$ satisfy the following,
\begin{align}
  &\bullet ~\sum_{j' \in [0,k]}\mxi_{i'j'} \in \Z_{\geq 0}\text{ for all } i' \in [1,i] ~~\bullet~\sum_{i'\in [\ell]}\mxi_{i'j'} \in \Z_{\geq 0} \text{ for all }j' \in [0,k]  \\
  %& \bullet ~\sum_{i' \in [\ell], j'\in [k]} m_{j'} \log r_{i'} \mxi_{i'j'} + \sum_{j' \in [k]}m_{j'} \log \rnew \vi{j'}  \geq \sum_{i' \in [\ell], j'\in [k]} m_{j'} \log r_{i'} \my_{i'j'}\\
  & \bullet \sum_{i' \in [\ell]} r_{i'} \sum_{j'\in [0,k]}\mxi_{i'j'} + \rnew \sum_{j' \in [0,k]} \vi_{j'}=\sum_{i' \in [\ell]} r_{i'} \sum_{j'\in [0,k]}\my_{i'j'} \label{eq:c1}\\
& \bullet ~\sum_{j' \in [0,k]}\vi_{j'} \in \Z_{\geq 0} ~~\bullet \sum_{i' \in [\ell]}\mxi_{i'j'}+\vi_{j'}=\sum_{i' \in [\ell]}\my_{i'j'} \text{ for all }j' \in [0,k] \label{eq:b1}\\
& \bullet ~\bg(\concat(\mxi,\vi)) \geq \exp(-\log n) \bg(\my)~. \label{eqy2}
\end{align}
The above expressions immediately proves conditions $(1,a)$, $(1,b)$, $(2)$ and in the remainder we prove condition $(3)$.

Consider $\myi = \concat(\mxi,\wwi)=\concat(\mxi,\vi,\wwimo)$ and $\myimo=\concat(\mximo,\wwimo)$, therefore we get that,
\begin{align}
    \bg(\myi)&=\bg(\concat(\mxi,\vi,\wwimo))=\bg(\concat(\mxi,\vi))+\bg(\wwimo),\\
    &\geq \exp(-O(\log n)) \bg(\my) +\bg(\wwimo)~,\\
    & \geq \exp(-O(\log n)) \bg(\mximo) + \bg(\wwimo),\\
    & \geq \exp(-O(\log n)) ( \bg(\mximo) + \bg(\wwimo) ),\\
    & = \exp(-O(\log n)) \bg(\concat(\mximo,\wwimo))=\exp(-O(\log n))\bg(\myimo)~.
\end{align}
The second and sixth inequalities hold as the function $\bg$ is separable in rows. The third and fourth inequalities follow from \Cref{eqy2} and \Cref{eqy1} respectively. 

All that remains is to show that $\myi \in \bZi$. As $\myi = \concat(\mxi,\vi,\wwimo)$ and $\myimo=\concat(\mximo,\wwimo)$, we have that for any $j' \in [0,k]$,
\begin{align*}
    \sum_{i' \in [\ell]} \myi_{i'j'}& =\sum_{i' \in [\ell]} (\mxi_{i'j'} + \vi_{j'} + \wwimo_{j'}) =\sum_{i' \in [\ell]} (\my_{i'j'}+\wwimo_{j'}),\\
    & =\sum_{i' \in [\ell]} (\mximo_{i'j'}+\wwimo_{j'})=\sum_{i' \in [\ell]} \myimo_{i'j'}=\phi_j~.
\end{align*}
The first and fourth equalities hold because of the definitions of $\myi$ and $\myimo$ respectively. The second and third inequalities follow from \Cref{eq:b1} and \Cref{eq:b2} respectively. The final equality holds because $\myimo \in \bZimo$ (assumption of the inductive step). Also note that,
\begin{align*}
    \sum_{i' \in [i+\ell]} \ri\sum_{j \in [0,k]}\myi_{i'j'}&=\sum_{i' \in [\ell]} \ri\sum_{j \in [0,k]}\mxi_{i'j'} + \rnew \sum_{j \in [0,k]} \vi_{j} + \sum_{i \in [|\bRimo|]}\ri  \sum_{j \in [0,k]} \wwi_{j}~,\\
    &=\sum_{i' \in [\ell]} \ri\sum_{j \in [0,k]}\my_{i'j'} + \sum_{i \in [|\bRimo|]}\ri  \sum_{j \in [0,k]} \wwi_{j}~,\\
    &=\sum_{i' \in [\ell]} \ri\sum_{j \in [0,k]}\mximo_{i'j'} + \sum_{i \in [|\bRimo|]}\ri  \sum_{j \in [0,k]} \wwi_{j}=\sum_{i' \in [\ell+i-1]} \ri\sum_{j \in [0,k]}\myimo_{i'j'} \leq 1~.
\end{align*}
The first and fourth equalities follow from the definitions of $\myi$ and $\myimo$. The second and third equalities hold from \Cref{eq:c1} and \Cref{eq:c2} respectively. The final inequality holds because $\myimo \in \bZimo$ (assumption of the inductive step). Therefore, we get that $\myi \in \bZi$ and we conclude the proof.
\end{proof}


==> algorithm.tex <==
Here we provide a proof sketch of \Cref{thm:algmain} and provide a description of the algorithm that proves it. The description of this algorithm is as follows.
\newcommand{\res}{\mathrm{residue}}
\newcommand{\create}{\mathrm{create}}
\newcommand{\roundi}{\mathrm{round\_i\_row}}
\newcommand{\pround}{\mathrm{partial\_round}}
\newcommand{\mxfinal}{\mx_{\mathrm{final}}}
\newcommand{\mxnew}{\mx_{\mathrm{new}}}
\newcommand{\mximo}{\mx^{(i-1)}}
\newcommand{\myimo}{\my^{(i-1)}}
\newcommand{\mxi}{\mx^{(i)}}
\newcommand{\myi}{\my^{(i)}}
\newcommand{\mylast}{\my^{(\ell-1)}}
\newcommand{\bRnew}{\textbf{\bR}_{\mathrm{new}}}
\newcommand{\rnew}{\textbf{r}_{\mathrm{new}}}
\newcommand{\bRfinal}{\textbf{\bR}_{\mathrm{final}}}
\newcommand{\bRi}{\textbf{R}^{(i)}}
\newcommand{\bRimo}{\textbf{R}^{(i-1)}}
\newcommand{\bZi}{\textbf{Z}^{\phi,frac}_{\bRi}}
\newcommand{\bZimo}{\textbf{Z}^{\phi,frac}_{\bRimo}}
\newcommand{\bZfinal}{\textbf{Z}^{\phi}_{\bRfinal}}
\newcommand{\mxtemp}{\mx_{\mathrm{temp}}}

\renewcommand{\vones}{\textbf{1}}
\newcommand{\vi}{\textbf{v}^{(i)}}
\newcommand{\vo}{\textbf{v}^{(1)}}
\newcommand{\vl}{\textbf{v}^{(\ell-1)}}
\newcommand{\ww}{\textbf{W}}
\newcommand{\wwi}{\textbf{W}^{(i)}}
\newcommand{\wwimo}{\textbf{W}^{(i-1)}}
\newcommand{\sparsify}{\mathrm{sparsify}}
\newcommand{\discretize}{\mathrm{discretize}}
%\newcommand{\res}{res}

\begin{algorithm}[H]
	\caption{ApproximatePML($\phi,\bR$)}
	\begin{algorithmic}[1]
	\State  $\mx=\argmax_{\mx' \in \bZfrac} \log \bg(\mx')$. \;
	\State $\mx=\sparsify(\mx)$.\;
	\State $\ww^{(0)}= [],\mx^{(0)}=\mx$, $\my^{(0)}=\mx$, $\bR^{(0)}=\bR$ and $\bRnew=\{\}$.\;
	\For{$i=1\dots \ell-1$.}
		 \State $(\my,j)=\pround(\mximo,i)$. \;
		 \State $(\mxi,\vi,\rnew)=\roundi(\my,j,i)$. \;
		 \State $\wwi=\concat(\wwimo,\vi)$ and $\bRnew=\bRnew \cup \{ \rnew\}$.\; 
		 \State $\myi=\concat(\mxi,\wwi)$ and $\bRi=\bRimo \cup \{ \rnew\}$.\;
		\EndFor
		\State $\mxfinal=\mylast$ and $\bRfinal=\bR^{(\ell-1)}$. \;
	\State Let $\bp'$ be the distribution with respect to $\mxfinal$ and $\bRfinal$ (See \Cref{defn:distX}).\;
	\State Return $\bq=\discretize(\bp',\phi,\bR)$\;
		%by assigning $(\bS \onevec)_{i}$ number of domain elements probability $\ri$ 
	%	\State \textbf{return} $\bpapprox\defeq \frac{\qext}{\|\qext\|_1}$.
		%\EndProcedure
	\end{algorithmic}
	\label{alg:main}
\end{algorithm}



% \begin{algorithm}
% 	\SetAlgoLined\DontPrintSemicolon
% 	\SetKwFunction{proc}{ApproximatePML}
% 	\SetKwProg{myproc}{Procedure}{}{}
% 	\myproc{\proc{$\phi,\bR$}}{
% 	\nl  $\mx=\argmax_{\mx' \in \bZfrac} \log \bg(\mx')$. \; \\
% 	\nl $\mx=\sparsify(\mx)$.\;\\
% 	\nl $\ww^{(0)}= [],\mx^{(0)}=\mx$, $\my^{(0)}=\mx$, $\bR^{(0)}=\bR$ and $\bRnew=\{\}$.\;\\
% 	\For{$i=1\dots \ell-1$.}{
% 		 $(\my,j)=\pround(\mximo,i)$. \;\\
% 		 $(\mxi,\vi,\rnew)=\roundi(\my,j,i)$. \;\\
% 		 $\wwi=\concat(\wwimo,\vi)$ and $\bRnew=\bRnew \cup \{ \rnew\}$.\; \\
% 		 $\myi=\concat(\mxi,\wwi)$ and $\bRi=\bRimo \cup \{ \rnew\}$.\;
% 		 }
% 		%\EndFor
% 		\nl $\mxfinal=\mylast$ and $\bRfinal=\bR^{(\ell-1)}$. \;\\
% 	\nl Let $\bp'$ be the distribution with respect to $\mxfinal$ and $\bRfinal$ (See \Cref{defn:distX}).\;\\
% 	\nl \KwRet $\bq=\discretize(\bp',\phi,\bR)$\;}
% 	\caption{Approximate PML algorithm}
% 	\label{alg:main}
% \end{algorithm}


Our algorithm includes various steps and in the following we will provide the guarantee of each step. We later use these guarantees to prove our final theorem (\Cref{thm:algmain}).
\begin{lem}[\cite{CSS19,ACSS20}]\label{lem:maximizer}
	Step 1 of the algorithm can be implemented in $\otilde(|\bR|~k^2)$ time and the maximizer $\mx$ satisfies: 
	$$\cphi \cdot \bg(\mx)\geq \expo{\bigO{-\min(k,|\bR|) \log n}} \max_{\bq \in \dsimplex}\probpml(\bq,\phi)~.$$
\end{lem}

\begin{lem}[Lemma 4.3 in \cite{ACSS20b}]\label{lem:sparse}
	For any $\mx \in \bZfrac$, the algorithm $\sparsify(\mx)$ runs in $\otilde(|\bR|~k^{\omega})$ time and returns a solution $\mx' \in \bZfrac$ such that, 
	$$\bg(\mx') \geq \bg(\mx) \text{ and } \big|\{i \in [\ell]~|~[\mx'\1]_{i}  > 0\}\big| \leq k+1~.$$
\end{lem}
Please refer to \cite{ACSS20b} for the description of the procedure $\sparsify$. The main usage of the procedure $\sparsify$ is that we can assume $|\bR| \leq k+1$ because we can ignore the zero rows of the matrix $\mx$.
\begin{lem}[Guarantees of the $i$'th iteration]\label{lem:iteri}
    For all $i \in [0,\ell-1]$, the following statements hold,
    \begin{enumerate}
        \item The matrix $\mxi \in \R_{\geq 0}^{\ell \times k}$ and satisfies the following inequalities:
        \begin{enumerate}
            \item $\sum_{i' \in [\ell]}\mxi_{i'j} \in \Z_{\geq 0} \text{ for all } j \in [0,k]$.
            \item $\sum_{j \in [k]}\mxi_{i'j} \in \Z_{\geq 0} \text{ for all } i' \in [1,i]$.
        \end{enumerate}
        \item The row vector $\vi \in \R_{\geq 0}^{[0,k]}$ has integral row sum, that is,
        $\sum_{j \in [0,k]} \vi_{j} \in \Z_{\geq 0}~.$
        \item The matrix $\myi \in \bZi$ and $\bg(\myi) \geq \exp(-\log n) \bg(\myimo)$.
    \end{enumerate}
\end{lem}
\begin{lem}\label{lem:final}
    The final variables $\mxfinal$ and $\bRfinal$ satisfy the following,
    \begin{itemize}
        \item $\mxfinal \in \bZfinal$.
        \item $\bg(\mxfinal) \geq \exp(-O(\min(k,|\bR|) \log n)) \bg(\mx)$~,
    \end{itemize}
    where $\ell'$ is the number of non-zero rows in the matrix $\mx$.
    %Furthermore the distribution $\bp'$ defined with respect to $\mxfinal$ and $\bRfinal$ (See \Cref{defn:distS}) satisfies,
    %$$\prob{\bp',\phi} \geq \exp(-O(\ell \log n)) \max_{\bq \in \dsimplex} \prob{\bq,\phi}~.$$
    %using the fact that, $\bg(\mx) \geq \exp(-O(\ell \log n)) \max_{\bq \in \dsimplex} \prob{\bq,\phi}$, we get that
    %Therefore $\bp'$ is the desired approximate PML distribution with respect to $\bR$.
\end{lem}
%\newcommand{\sink}{\mathrm{sink}}
\newcommand{\mq}{\textbf{Q}}
We also need the following discretization lemma, that helps us return a pseudo distribution that belongs to $\dsimplex$.
\begin{lem}\label{lem:disc}
    The function $\discretize$ takes input a distribution $\bp \in \simplex$ with $\ell'$ distinct probability values, a profile $\phi$, a discretization set of the form $\bR=\{\frac{1}{2n^2},\dots,\frac{1}{2n^2}(1+\alpha)^i,\dots,1 \}$ for some $\alpha \in (0,1)$ and outputs a pseudo distribution $\bq \in \dsimplex$ such that,
    \begin{equation}
        \prob{\frac{\bq}{\|\bq\|_1},\phi} \geq \exp(-O(\min(k,|\bR|)+\min(k,\ell') + \alpha^2n) \log n) \prob{\bp,\phi}.
    \end{equation}
\end{lem}
In \Cref{subsec:one}, we use the guarantees stated above for each step of \Cref{alg:main} to prove \Cref{thm:algmain}. The description of the function $\discretize$ is specified in the proof of \Cref{lem:disc}. We need the guarantees of sub routines $\pround$ and $\roundi$ to prove \Cref{lem:iteri}. A description for sub routines $\pround$ and $\roundi$ along with the guarantees are provided in \Cref{subsec:partial} and \Cref{subsec:roundi} respectively. We defer the proof of all these results to appendix.

\subsection{Proof of \Cref{thm:algmain}}\label{subsec:one}
\begin{proof}
As $\mxfinal \in \bZfinal$, by definition \Cref{defn:distX} and \Cref{pmlprob:approx} we get that,
\begin{align*}
\prob{\bp',\phi} &\geq \exp(-O( \min(k,|\bRfinal|) \log n)) \cphi \bg(\mxfinal)~,\\
&\geq \exp(-O( (\min(k,|\bRfinal|)+\min(k,|\bR|)) \log n)) \cphi \bg(\mx)~,\\
& \geq \exp(-O( \min(k,|\bR|) \log n)) \cphi \max_{\mx' \in \bZ} \bg(\mx')~,\\    
& \geq \exp(-O( \min(k,|\bR|) \log n)) \max_{\bq \in \dsimplex}\probpml(\bq,\phi)~.
\end{align*}
In the second inequality we used the second condition of \Cref{lem:final}. In the third inequality we used the definition of $\mx$ (Step 1) and $|\bRfinal| \leq |\bR|+\ell \leq 2 \bR$. In the final inequality we used \Cref{lem:maximizer}.

Note that we don't have a complete proof yet, as we need a distribution that approximately maximizes $\max_{\bq \in \dsimplex}\probpml(\frac{\bq}{\|\bq\|_1},\phi)$ instead of just $\max_{\bq \in \dsimplex}\probpml({\bq},\phi)$. To provide a distribution with such a guarantee we do the following. For any pseudo distribution $\bq \in \dsimplex$, note that its $\ell_1$ norm satisfies: $\rmin \leq \|\bq\|_1 \leq 1$, and for any constant $c>0$, let $c\cdot \bR \defeq \{c \cdot \ri ~|~\ri \in \bR \}$. Then note that,
\begin{equation}\label{eq:a1}
    \max_{\bq \in \dsimplex}\probpml(\frac{\bq}{\|\bq\|_1},\phi) = \max_{c \in [1,1/\rmin]_{\R}}~~ \max_{\bq \in \Delta^{\bX}_{c\cdot \bR}}\probpml(\bq,\phi)~.
\end{equation}
The above equality holds as the maximizer $\bq^*$ of the left hand side belongs to $\bq^{*} \in \Delta^{\bX}_{(1/\| \bq*\|_1)\cdot \bR}$. Let $C\defeq \{(1+\beta)^i \}_{i \in [a]}$ for some $\beta \in o(1)$, where $a \in O(\frac{1}{\beta}\log (1/\rmin))$ is such that $\rmin (1+\beta)^a=1$. For any constant $c \in [1,1/\rmin]_{\R}$, note that there exists a constant $c' \in C$ such that $c(1-\beta) \leq c' \leq c $. Furthermore, for any distribution $\bq \in \dsimplex$ with $\|\bq\|_1=1/c$, note that the distribution $\bq'=c' \bq \in \Delta^{\bX}_{c'\cdot \bR}$ and satisfies,
\begin{align*}
\probpml(\frac{\bq}{\|\bq\|_1},\phi) =\probpml({c \cdot \bq},\phi)=\probpml(\frac{c}{c'} \bq',\phi)
=\left(\frac{c}{c'}\right)^n\probpml({\bq'},\phi)~.
\end{align*}
Therefore we get that,
$$\probpml({\bq'},\phi) = \left(\frac{c'}{c}\right)^n \probpml(\frac{\bq}{\|\bq\|_1},\phi) \geq (1-\beta)^n\probpml(\frac{\bq}{\|\bq\|_1},\phi) \geq \exp(-2\beta n)\probpml(\frac{\bq}{\|\bq\|_1},\phi) ~.$$
The above analysis combined with \Cref{eq:a1} gives,
\begin{equation}
    \max_{c \in C}~~ \max_{\bq \in \Delta^{\bX}_{c\cdot \bR}}\probpml(\bq,\phi) \geq \exp(-2\beta n)\max_{\bq \in \dsimplex}\probpml(\frac{\bq}{\|\bq\|_1},\phi).
\end{equation}
For each $c$, our algorithm (\Cref{alg:main}) returns a distribution $\bp_{c}$ that satisfies,
$$\prob{\bp_c,\phi} \geq \exp(-O( \min(k,|\bR|) \log n)) \max_{\bq \in \Delta^{\bX}_{c\cdot \bR}}\probpml(\bq,\phi)~.$$
In the above inequality we used $|\bR|=|c\cdot \bR|$. Let $\bp^{*}$ be the distribution with maximum objective value to our convex program and note that it satisfies,
$$\prob{\bp^*,\phi} \geq \exp(-O( \min(k,|\bR|) \log n)-2 \beta n) \max_{\bq \in \dsimplex}\probpml(\frac{\bq}{\|\bq\|_1},\phi)~.$$
Choose $\beta=\frac{\min(k,|\bR|)}{n}$, we get that,
$$\prob{\bp^*,\phi} \geq \exp(-O( \min(k,|\bR|) \log n)) \max_{\bq \in \dsimplex}\probpml(\frac{\bq}{\|\bq\|_1},\phi)~.$$
Finally, note that each of our distributions $\bp_c$ have the number of distinct probability values upper bounded by $2|\bR|$. Therefore, applying \Cref{lem:disc}, we get a pseudo distribution $\bq \in \dsimplex$ with the desired guarantees and we are done. The running time of our algorithm is $O(|C|\mathcal{T}_{1}) \in O(\frac{n}{\min(k,|\bR|)} \cdot \mathcal{T}_{1})$, where $\mathcal{T}_1$ is the time to implement \Cref{alg:main}. As all the steps of \Cref{alg:main} are polynomial in $n$, our final running time is polynomial in $n$ and we conclude the proof.

\end{proof}

\subsection{Description and guarantees of $\pround$}\label{subsec:partial}
Here we provide the description of $\pround$ and its guarantees are summarized in \Cref{lem:partial-round}. 

\begin{algorithm}[H]
	\caption{$\pround(\mx,i)$}
	\begin{algorithmic}[1]
	\State $\mtz=\msplit{\mx}{i}$. \;
	\State $(\mw,j)=\proundx(\mtz,i+1)$. \;
	\State $\my=\mcombine{\mw}{i}$. \;
	\State Return $(\my,j)$. \;
	\end{algorithmic}
	\label{alg:pround}
\end{algorithm}



% \begin{algorithm}[H]
%     \SetAlgoLined\DontPrintSemicolon
% 	\SetKwFunction{proc}{$\pround$}
% 	\SetKwProg{myproc}{Procedure}{}{}
% 	\myproc{\proc{$\mx,i$}}{
% 	\nl $\mtz=\msplit{\mx}{i}$. \;\\
% 	\nl $(\mw,j)=\proundx(\mtz,i+1)$. \;\\
% 	\nl $\my=\mcombine{\mw}{i}$. \;\\
% 	\nl Return $(\my,j)$. \;
%     }
% 	\caption{$\pround(\mx,i)$} \label{alg:pround}
% \end{algorithm}


\begin{lem}\label{lem:partial-round}
The algorithm $\pround$ takes in inputs $\mx \in \R^{\ell \times [0,k]}_{\geq 0}$ and $i \in [\ell-1]$ that satisfies the following,
$\sum_{j \in [0,k]}\mx_{i'j} \in \Z_{\geq 0} \text{ for all } i'\in [1,i-1] \text{ and }\sum_{i' \in [\ell]} \mx_{i'j} \in \Z_{\geq 0} \text{ for all }j\in [0,k]$,
and outputs a matrix $\my \in \R_{\geq 0}^{\ell \times [0,k]}$ such that $\|\my-\mx\|_1\leq O(1)$ and an index $j'$ such that,
\begin{align}
  & \bullet ~\sum_{i \in [\ell], j\in [k]} m_j \log r_i \my_{ij} \geq \sum_{i \in [\ell], j\in [k]} m_j \log r_i \mx_{ij} ~~ \bullet ~\sum_{i \in [\ell]}\my_{ij}=\sum_{i \in [\ell]}\mx_{ij} \text{ for all } j \in [0,k]\\
  &\bullet ~\sum_{j \in [k]}\my_{ij} =\sum_{j \in [k]}\mx_{ij} \text{ for all } i \in [\ell]
  ~~\bullet ~\my_{ij'} \geq o \text{ and } \sum_{i'=1}^{i-1} \my_{i'j'}+\my_{ij'}-o \in \Z_{\geq 0},
\end{align}
where $o=\sum_{j \in [0,k]}\mx_{ij} - \lfloor \sum_{j \in [0,k]}\mx_{ij} \rfloor$. Furthermore, the running time of the algorithm is $O()$. \kk{Fill in the running time.}
\end{lem}
Our algorithm invokes several subroutines and in the following we provide description for each of these and also state their guarantees. The subroutine $\proundx$ provides an algorithm that proves the \Cref{lem:partial-round} in the special case of $[\mx \onevec]_i \in [0,1)$. The description of this subroutine and its guarantees are stated below. For convenience, we first introduce some new notation.
\paragraph{Notation:} For any matrix $\mx \in \R_{\geq 0}^{\ell \times [0,k]}$ and indices $i_1,i_2,j_1,j_2$, we define $\summx{i_1}{i_2}{j_1}{j_2} \defeq \sum_{i=i_1}^{i_2}\sum_{j=j_1}^{j_2}\mx_{ij}$ and say $(i,j)\in \twodinterval{i_1}{i_2}{j_1}{j_2}$ if $i_1\leq i\leq i_2$ and $j_1\leq j\leq j_2$. Therefore, $\summx{i_1}{i_2}{j_1}{j_2} = \sum_{(i,j)\in \twodinterval{i_1}{i_2}{j_1}{j_2}}\mx_{ij}$. Also note that when $i_1\geq i_2+1$ or $j_1\geq j_2+1$, we are summing over a empty set and $\summx{i_1}{i_2}{j_1}{j_2}\defeq 0$.
%
The description of our subroutine $\proundx$ is as follows.
\begin{algorithm}[H]
	\caption{$\proundx(\mx,i)$}
	\begin{algorithmic}[1]
	\State $j=\min\{r:  \mx(1:\ell, 0:r) > \mx(1:i-1, 0:k)$. \;
	\State $t=\mx(1:i-1, 0:k) -\mx(1:\ell, 0:j-1)$.\;
    \State $\my=\mx$.\;
	\State $\trans{\my}{\summy{i}{i}{0}{j-1}}{\transpara{1}{i-1}{i}{i}{0}{j-1}{j}{k}}$. \label{alg:prs:1}\;
	\If{ $\summy{1}{i-1}{j}{j}\geq t$ }
	    \State $v=\summy{1}{i-1}{j}{j}-\left\lfloor\summy{1}{i-1}{j}{j}\right\rfloor$. \;
	    \State $\trans{\my}{\min\left\{v+1 , \summy{1}{i-1}{j}{j}-t\right\}}{\transpara{1}{i-1}{i+1}{\ell}{0}{j-1}{j}{j}}$. \label{alg:prs:2} \;
	\Else
	    \State $v=\left\lceil\summy{1}{i-1}{j}{j}\right\rceil - \summy{1}{i-1}{j}{j}$. \;
	    \State $\trans{\my}{v}{\transpara{1}{i-1}{i}{\ell}{j}{j}{j+1}{k}}$. \label{alg:prs:3} \;
	   \EndIf
	\State $\trans{\my}{\summy{i}{i}{j+1}{k}}{\transpara{i}{i}{i+1}{\ell}{j}{j}{j+1}{k}}$. \label{alg:prs:4} \;
	\State Return $(\my,j)$. \label{alg:prs:5} \;
	\end{algorithmic}
	\label{alg:proundx}
\end{algorithm}


\begin{tikzpicture} % pic for partial_round
\coordinate (p1) at (0,0);
\coordinate (p2) at ([xshift=5cm] p1);
\coordinate (p3) at ([xshift=5cm] p2);
\coordinate (p33) at ([yshift=-5cm] p2);
\coordinate (p4) at ([yshift=-5cm] p3);
%
\coordinate (o1) at ([xshift=3cm,yshift=3cm] p1);
\coordinate (o2) at ([xshift=3cm,yshift=3cm] p2);
\coordinate (o3) at ([xshift=3cm,yshift=3cm] p3);
\coordinate (o33) at ([xshift=3cm,yshift=3cm] p33);
\coordinate (o4) at ([xshift=3cm,yshift=3cm] p4);
%
\coordinate (q1) at ([xshift=3.25cm] p1);
\coordinate (q2) at ([xshift=3.25cm] p2);
\coordinate (q22) at ([yshift=-1.75cm] p2);
\coordinate (q3) at ([yshift=-1.75cm] p3);
\coordinate (q33) at ([xshift=3.25cm] p33);
\coordinate (q4) at ([xshift=3.25cm] p2);
%
\coordinate (r1) at ([xshift=1.5cm,yshift=1.5cm] q1);
\coordinate (r2) at ([xshift=1.5cm,yshift=1.5cm] q2);
\coordinate (r22) at ([xshift=1.5cm,yshift=1.5cm] q22);
\coordinate (r3) at ([xshift=1.5cm,yshift=1.5cm] q3);
\coordinate (r33) at ([xshift=1.5cm,yshift=1.5cm] q33);
%
\draw (p1) rectangle (o1);
\draw (p2) rectangle (o2);
\draw (p3) rectangle (o3);
\draw (p33) rectangle (o33);
\draw (p4) rectangle (o4);
%
\draw (q1) rectangle (r1);
\draw (q2) rectangle (r2);
\draw (q22) rectangle (r22);
\draw (q3) rectangle (r3);
\draw (q33) rectangle (r33);
%
\draw [help lines, shift=(p1)]
{
(0,1)--(3,1) 
(0,2)--(3,2)
(1,0)--(1,3)
(2,0)--(2,3)
};
\draw [help lines, shift=(p2)]
{
(0,1)--(3,1) 
(0,2)--(3,2)
(1,0)--(1,3)
(2,0)--(2,3)
};
\draw [help lines, shift=(p3)]
{
(0,1)--(3,1) 
(0,2)--(3,2)
(1,0)--(1,3)
(2,0)--(2,3)
};
\draw [help lines, shift=(p33)]
{
(0,1)--(3,1) 
(0,2)--(3,2)
(1,0)--(1,3)
(2,0)--(2,3)
};
\draw [help lines, shift=(p4)]
{
(0,1)--(3,1) 
(0,2)--(3,2)
(1,0)--(1,3)
(2,0)--(2,3)
};
%
\draw[->, shift=(p1)]  (3.2,2) --  (4.8,2);
\draw[->, shift=(p2)]  (3.2,2) --  (4.8,2);
\draw[->, shift=(p33)]  (3.2,2) --  (4.8,2);
\draw[->, shift=(p2)]  (2,-0.2) --  (2,-1.8);
\draw[->, shift=(p3)]  (2,-0.2) --  (2,-1.8);
%
\node at ([xshift=4cm,yshift=2.3cm] p1)  { Step \ref{alg:prs:1}};
\node at ([xshift=4cm,yshift=2.3cm] p2)  { Step \ref{alg:prs:2}};
\node at ([xshift=4cm,yshift=2.3cm] p33)  { Step \ref{alg:prs:4}};
\node at ([xshift=2.7cm,yshift=-1cm] p2)  { Step \ref{alg:prs:3}};
\node at ([xshift=2.7cm,yshift=-1cm] p3)  { Step \ref{alg:prs:4}};
%
\draw [help lines, shift=(q1)]
{
(0,0.5)--(1.5,0.5) 
(0,1)--(1.5,1)
(0.5,0)--(0.5,1.5)
(1,0)--(1,0.5)
};
\node at ([xshift=0.25cm,yshift=1.25cm] q1) {$+$};
\node at ([xshift=0.25cm,yshift=0.75cm] q1) {$-$};
\node at ([xshift=1cm,yshift=1.25cm] q1) {$-$};
\node at ([xshift=1cm,yshift=0.75cm] q1) {$+$};
\draw [help lines, shift=(q2)]
{
(0,0.5)--(1.5,0.5) 
(0,1)--(1.5,1)
(0.5,0)--(0.5,1.5)
(1,0)--(1,1.5)
};
\node at ([xshift=0.25cm,yshift=1.25cm] q2) {$+$};
\node at ([xshift=0.25cm,yshift=0.25cm] q2) {$-$};
\node at ([xshift=0.75cm,yshift=1.25cm] q2) {$-$};
\node at ([xshift=0.75cm,yshift=0.25cm] q2) {$+$};
\draw [help lines, shift=(q22)]
{
(0,0.5)--(0.5,0.5) 
(0,1)--(1.5,1)
(0.5,0)--(0.5,1.5)
(1,0)--(1,1.5)
};
\node at ([xshift=0.75cm,yshift=1.25cm] q22) {$+$};
\node at ([xshift=0.75cm,yshift=0.5cm] q22) {$-$};
\node at ([xshift=1.25cm,yshift=1.25cm] q22) {$-$};
\node at ([xshift=1.25cm,yshift=0.5cm] q22) {$+$};
\draw [help lines, shift=(q3)]
{
(0,0.5)--(1.5,0.5) 
(0,1)--(1.5,1)
(0.5,0)--(0.5,1.5)
(1,0)--(1,1.5)
};
\node at ([xshift=0.75cm,yshift=0.75cm] q3) {$+$};
\node at ([xshift=0.75cm,yshift=0.25cm] q3) {$-$};
\node at ([xshift=1.25cm,yshift=0.75cm] q3) {$-$};
\node at ([xshift=1.25cm,yshift=0.25cm] q3) {$+$};
\draw [help lines, shift=(q33)]
{
(0,0.5)--(1.5,0.5) 
(0,1)--(1.5,1)
(0.5,0)--(0.5,1.5)
(1,0)--(1,1.5)
};
\node at ([xshift=0.75cm,yshift=0.75cm] q33) {$+$};
\node at ([xshift=0.75cm,yshift=0.25cm] q33) {$-$};
\node at ([xshift=1.25cm,yshift=0.75cm] q33) {$-$};
\node at ([xshift=1.25cm,yshift=0.25cm] q33) {$+$};
%
\node at ([xshift=0.5cm,yshift=1.5cm] p2) {$=0$};
\node at ([xshift=0.5cm,yshift=1.5cm] p3) {$=0$};
\node at ([xshift=0.5cm,yshift=1.5cm] p33) {$=0$};
\node at ([xshift=0.5cm,yshift=1.5cm] p4) {$=0$};
\node at ([xshift=1.5cm,yshift=2.5cm] p3) {$\in \Z_{\geq 0}$};
\node at ([xshift=1.5cm,yshift=2.5cm] p33) {$\in \Z_{\geq 0}$};
\node at ([xshift=1.5cm,yshift=2.5cm] p4) {$\in \Z_{\geq 0}$};
\node at ([xshift=2.5cm,yshift=1.5cm] p4) {$=0$};

\end{tikzpicture}






% \begin{algorithm}[H]
%     \SetAlgoLined\DontPrintSemicolon
% 	\SetKwFunction{proc}{$\proundx$}
% 	\SetKwProg{myproc}{Procedure}{}{}
% 	\myproc{\proc{$\mx,i$}}{
% 	\nl $j=\min\{r:\sum_{j'=0}^{r}\sum_{i'\in [\ell]}\mx_{i'j'} > \sum_{i'=1}^{i-1}\sum_{j\in [0,k]}\mx_{i'j'}\}$. \;\\
% 	\nl $t=\sum_{i'=1}^{i-1}\sum_{j\in [0,k]}\mx_{i'j'} - \sum_{j'=0}^{j-1}\sum_{i'\in [\ell]}\mx_{i'j'}$.\;\\
%     \nl $\my=\mx$.\;\\
% 	\nl $\trans{\my}{\summy{i}{i}{0}{j-1}}{\transpara{1}{i-1}{i}{i}{0}{j-1}{j}{k}}$. \label{alg:prs:1}\;\\
% 	\eIf{ $\summy{1}{i-1}{j}{j}\geq t$ }
% 	{
% 	    \nl $v=\summy{1}{i-1}{j}{j}-\left\lfloor\summy{1}{i-1}{j}{j}\right\rfloor$. \;\\
% 	    \nl $\trans{\my}{\min\left\{v+1 , \summy{1}{i-1}{j}{j}-t\right\}}{\transpara{1}{i-1}{i+1}{\ell}{0}{j-1}{j}{j}}$. \label{alg:prs:2} \;
% 	}
% 	{
% 	    \nl $v=\left\lceil\summy{1}{i-1}{j}{j}\right\rceil - \summy{1}{i-1}{j}{j}$. \;\\
% 	    \nl $\trans{\my}{v}{\transpara{1}{i-1}{i}{\ell}{j}{j}{j+1}{k}}$. \label{alg:prs:3} \;
% 	}
% 	\nl $\trans{\my}{\summy{i}{i}{j+1}{k}}{\transpara{i}{i}{i+1}{\ell}{j}{j}{j+1}{k}}$. \label{alg:prs:4} \;\\
% 	\nl Return $(\my,j)$. \label{alg:prs:5}} \;
% 	\caption{$\proundx(\mx,i)$} \label{alg:proundx}
% \end{algorithm}
In the above lemma, we have defined an operation called $\transname$, the description of this operation is specified in the proof of \Cref{lem:trans} and due to space constraints we defer its proof to appendix. As discussed earlier, following is the guarantee of subroutine $\proundx$.
\begin{lem}[Guarantee of $\proundx$]\label{lem:proundx}
The algorithm $\proundx$ takes in inputs $\mx \in \R^{\ell \times [0,k]}_{\geq 0}$ and $i \in [1,\ell-1]$ that satisfy the conditions of \Cref{lem:partial-round} with an additions assumption that $\sum_{j' \in [0,k]}\mx_{ij'} \in [0,1)$ and outputs a matrix $\my \in \R_{\geq 0}^{\ell \times [0,k]}$ and an index $j$ that satisfy the guarantees of \Cref{lem:partial-round}. Furthermore, the running time of this procedure is $O(\ell k)$.
% The algorithm $\proundx$ takes in inputs $\mx \in \R^{\ell \times [0,k]}_{\geq 0}$ and $i \in [1,\ell-1]$ that satisfies the following, 
% $$\sum_{j' \in [0,k]}\mx_{i'j'} \in \Z_{\geq 0} \text{ for all } i'\in [1,i-1] , ~\sum_{i' \in [\ell]} \mx_{i'j'} \in \Z_{\geq 0} \text{ for all }j'\in [0,k] \text{ and }\sum_{j' \in [0,k]}\mx_{ij'} \in [0,1)~,$$
% and outputs a matrix $\my \in \R_{\geq 0}^{\ell \times [0,k]}$ such that $\|\my-\mx\|_1\leq O(1)$ and an index $j$ such that,
% \begin{align}
%   & \bullet ~\sum_{i' \in [\ell], j'\in [0,k]} m_{j'} \log r_{i'} \my_{i'j'} \geq \sum_{i' \in [\ell], j'\in [0,k]} m_{j'} \log r_{i'} \mx_{i'j'}    \\ 
%   & \bullet ~\sum_{i' \in [\ell]}\my_{i'j'}=\sum_{i' \in [\ell]}\mx_{i'j'} \text{ for all } j' \in [0,k]\\
%   &\bullet ~\sum_{j' \in [0,k]}\my_{i'j'} =\sum_{j' \in [0,k]}\mx_{i'j'} \text{ for all } i' \in [\ell]
%   ~~\bullet ~\my_{ij} = \sum_{j' \in [0,k]}\mx_{ij'} \text{ and } \sum_{i'=1}^{i-1} \my_{i'j} \in \Z_{\geq 0}.
% \end{align}
% Furthermore, the running time of the algorithm is $O(\ell k)$.
\end{lem}
To extend the above algorithm for the general case, we define simple operations $\msplitname$ and $\mcombinename$ that we define next. Intuitively, the operation $\mcombinename$ combines $i$-th and $(i+1)$-th rows by adding them up, and $\msplitname$ splits $i$-th row into two rows so that the summation of one row is an integer and the summation of the other row is less than one.
\begin{defn}[Combine]
For any $\mw \in \R_{\geq 0}^{(\ell+1) \times [0,k]}$ and $t\in [1,\ell]$, $\my\defeq \mcombine{\mw}{t}\in \R_{\geq 0}^{\ell \times [0,k]}$ is defined as follows,
\begin{align*}
    \my_{i,j}=
    \begin{cases}
    \mw_{i,j} & i\leq t-1    \\
    \mw_{i,j}+\mw_{(i+1),j} & i= t    \\
    \mw_{(i+1),j} & i\geq t+1 
    \end{cases}
\end{align*}
\end{defn}

\begin{tikzpicture} % pic for combine
\draw (0,0) rectangle (3,4);
\draw [help lines] (0,1) -- (3,1);
\draw [help lines] (0,2) -- (3,2);
\draw [help lines] (0,3) -- (3,3);
\node  at (1.5,3.5) {$\mw_{[1:i-1],[0:k]}$} ;
\node  at (1.5,2.5) {$\mw_{[i:i],[0:k]}$} ;
\node  at (1.5,1.5) {$\mw_{[i+1:i+1],[0:k]}$} ;
\node  at (1.5,0.5) {$\mw_{[i+2:\ell+1],[0:k]}$} ;
%
\draw (5,0.5) rectangle (8,3.5);
\draw [help lines] (5,1.5) -- (8,1.5);
\draw [help lines] (5,2.5) -- (8,2.5);
\node  at (6.5,3) {$\my_{[1:i-1],[0:k]}$} ;
\node  at (6.5,2) {$\my_{[i:i],[0:k]}$} ;
\node  at (6.5,1) {$\my_{[i+1:\ell],[0:k]}$} ;
%
\draw[->] (3,3.5)--(5,3);
\draw[->] (3,2.5)--(5,2);
\draw[->] (3,1.5)--(5,2);
\draw[->] (3,0.5)--(5,1);
\end{tikzpicture}




\begin{defn}[Split]
Let $\mx \in \R_{\geq 0}^{\ell \times [0,k]}$, $r(t):=\sum_{j\in [0,k]}\mx_{tj}$ and $s(t):=\min\{ j:\sum_{j'\leq j}\mx_{tj'}\geq \lfloor r(t)\rfloor  \}$.
We define $\msplit{\mx}{t}$ to be $\mtz\in \R_{\geq 0}^{(\ell+1) \times [0,k]}$ where,
\begin{align*}
    \mtz_{i,j}= \mx_{i,j}, ~~ i\leq t-1    \quad \quad \quad \quad \mtz_{i,j}= \mx_{(i-1),j},  i\geq t+2
\end{align*}
\begin{align*}
     \mtz_{t,j}=
    \begin{cases}
      \mx_{t,j}, & j<s(t) \\
        \lfloor r(t)\rfloor - \sum_{j'\leq j-1}\mx_{t,j'}, & j=s(t)\\
        0, & j>s(t)
    \end{cases}
    \quad \quad 
    \mtz_{t+1,j}=
    \begin{cases}
    0,  & j<s(t)    \\
     \sum_{j'\leq j}\mx_{t,j'} - \lfloor r(t)\rfloor, &  j=s(t)\\
    \mx_{t,j}, & j>s(t)
    \end{cases}
\end{align*}
% \begin{align*}
%     \mtz_{i,j}=
%     \begin{cases}
%     \mx_{i,j}, ~~ i\leq t-1  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \mx_{t,j}, ~~ i= t, j<s(t)    \\
%     \lfloor r(t)\rfloor - \sum_{j'\leq j-1}\mx_{t,j'}, ~~ i= t, j=s(t)    ~~~~~~~~~~~~~~~~~
%     0, ~~ i= t, j>s(t)    \\
%     \sum_{j'\leq j}\mx_{t,j'} - \lfloor r(t)\rfloor, ~~ i= t+1, j=s(t)  ~~~~~~~~~~~~~~
%     0, ~~ i= t+1, j<s(t)    \\
%     \mx_{t,j}, ~~ i= t+1, j>s(t)    ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%     \mx_{(i-1),j},  i\geq t+2 
%     \end{cases}
% \end{align*}
 \end{defn}
 
 

\begin{tikzpicture} % pic for split
\draw (0,0) rectangle (3,3);
\draw [help lines] (0,1) -- (3,1);
\draw [help lines] (0,2) -- (3,2);
\node  at (1.5,2.5) {$\mx_{[1:i-1],[0:k]}$} ;
\node  at (1.5,1.5) {$\mx_{[i:i],[0:k]}$} ;
\node  at (1.5,0.5) {$\mx_{[i+1:\ell],[0:k]}$} ;
%
\draw (5,-0.5) rectangle (8,3.5);
\draw [help lines] (5,0.5) -- (8,0.5);
\draw [help lines] (5,1.5) -- (8,1.5);
\draw [help lines] (5,2.5) -- (8,2.5);
\node  at (6.5,3) {$\mtz_{[1:i-1],[0:k]}$} ;
\node  at (6.5,2) {$\mtz_{[i:i],[0:k]}$} ;
\node  at (6.5,1) {$\mtz_{[i+1:i+1],[0:k]}$} ;
\node  at (6.5,0) {$\mtz_{[i+2:\ell+2],[0:k]}$} ;
%
\draw[->] (3,2.5)--(5,3);
\draw[->] (3,1.5)--(5,2);
\draw[->] (3,1.5)--(5,1);
\draw[->] (3,0.5)--(5,0);
\end{tikzpicture}

 
 
We remark that $\mtz$ has the following properties: 1) $\mcombine{\mtz}{t}=\mx$, 2) $\sum_{j\in [0,k]}\mtz_{tj}=\lfloor r(t) \rfloor$, 3) $\sum_{j\in [0,k]}\mtz_{(t+1),j}=r(t)-\lfloor r(t) \rfloor$, which is a real number in $[0,1)$.

\subsection{Description and guarantees of $\roundi$}\label{subsec:roundi}
Here we provide a description of the subroutine $\roundi$.

\begin{algorithm}[H]
	\caption{$\roundi(\my,j,i,o)$}
	\begin{algorithmic}[1]
	    \State Let matrix $\mx \in \R_{\geq 0}^{\ell \times [0,k]}$ and vector $v \in \R_{\geq 0}^{[0,k]}$ as follows.\;
	    \State Assign $\mx_{i'j'}=\my_{i'j'}$ for all $i' \in [\ell], ~j'\in [0,k] \text{ and }j' \neq j$.\;
		\State Assign $\mx_{i'j}=\my_{i'j}$ for all $i' \in [1,i-1]$.\;
		\State Assign $w_i=o$ and $\mx_{ij}=\my_{ij}-w_i$.\;\label{algs:assignx=y-o}
		\State Assign $\res=1-o$ and $\rnew=\ri\cdot w_i$.\;
		\For{$i'=i+1\dots \ell$}
		\State Let $w_{i'}=\min(\my_{i'j},\res)$.\;
		\State $\mx_{i'j}=\my_{i'j}-w_{i'}$.\;\label{algs:assignx=y-w} 
		\State $\rnew=\rnew+\textbf{r}_{i'} \cdot w_{i'}$.\; 
		\State $\res=\res-w_{i'}$.\; 
		\If{$\res=0$}
		\State exit the for loop.
		\EndIf
		\EndFor
		\State Assign $v_{j}=1$ and $v_{j'}=0$ for all $j' \in [0,k]$ and $j' \neq j$.\; \label{algs:assignv}
		\State Return $(\mx,v,\rnew)$. \;
	\end{algorithmic}
	\label{alg:final_temp}
\end{algorithm}

% \begin{algorithm}[H]
% 	\SetAlgoLined\DontPrintSemicolon
% 	\SetKwFunction{proc}{$\roundi$}
% 	\SetKwProg{myproc}{Procedure}{}{}
% 	\myproc{\proc{$\my,j,i,o$}}{
% 	\nl Let matrix $\mx \in \R_{\geq 0}^{\ell \times [0,k]}$ and vector $v \in \R_{\geq 0}^{[0,k]}$ as follows.\;\\ 
% 		\nl Assign $\mx_{i'j'}=\my_{i'j'}$ for all $i' \in [\ell], ~j'\in [0,k] \text{ and }j' \neq j$.\;\\ 
% 		\nl Assign $\mx_{i'j}=\my_{i'j}$ for all $i' \in [1,i-1]$.\;\\ 
% 		\nl Assign $w_i=o$ and $\mx_{ij}=\my_{ij}-w_i$.\;\label{algs:assignx=y-o}\\ 
% 		\nl Assign $\res=1-o$ and $\rnew=\ri\cdot w_i$.\;\\ 
% 		\For{$i'=i+1\dots \ell$}
% 		{
% 		\nl Let $w_{i'}=\min(\my_{i'j},\res)$.\;\\ 
% 		\nl $\mx_{i'j}=\my_{i'j}-w_{i'}$.\;\label{algs:assignx=y-w}\\ 
% 		\nl $\rnew=\rnew+\textbf{r}_{i'} \cdot w_{i'}$.\;\\ 
% 		\nl $\res=\res-w_{i'}$.\;\\ 
% 		\If{$\res=0$}
% 		{
% 		\nl exit the for loop.
% 		}
% 		}
% 		\nl Assign $v_{j}=1$ and $v_{j'}=0$ for all $j' \in [0,k]$ and $j' \neq j$.\; \label{algs:assignv} \\ 
% 		\nl \KwRet Return $(\mx,v,\rnew)$. \;}
% 	\caption{Rounds the $i$th row}
% 	\label{alg:final_temp}
% \end{algorithm}
The guarantees of the above algorithm are summarized in the lemma below.
\begin{lem}\label{lem:roundi}
    The algorithm $\roundi$ takes in inputs $\my \in \R_{\geq 0}^{\ell \times [0,k]}$, an column index $j \in [0,k]$, a row index $i \in [\ell-1]$ and a scalar $o\in (0,1)$ such that, $\sum_{j' \in [0,k]}\my_{i'j'} \in \Z_{\geq 0} \text{ for all } i' \in [i-1]$, $\sum_{i'\in [\ell]}\my_{i'j'} \in \Z_{\geq 0} \text{ for all }j' \in [0,k]$, $\my_{ij} \geq o$ and $\sum_{i'=1}^{i-1} \my_{i'j}+\my_{ij}-o \in \Z_{\geq 0}$,
%     \begin{align}
%   &\bullet ~\sum_{j' \in [0,k]}\my_{i'j'} \in \Z_{\geq 0} \text{ for all } i' \in [i-1]
%   ~~\bullet ~ \sum_{i'\in [\ell]}\my_{i'j'} \in \Z_{\geq 0} \text{ for all }j' \in [0,k]\\
%   & \bullet ~\my_{ij} \geq o \text{ and } \sum_{i'=1}^{i-1} \my_{i'j}+\my_{ij}-o \in \Z_{\geq 0},
% \end{align}
where $o=\sum_{j \in [0,k]}\my_{ij} - \lfloor \sum_{j \in [0,k]}\my_{ij} \rfloor$. Outputs a matrix $\mx \in \R_{\geq 0}^{\ell \times [0,k]}$, a new probability value $\rnew \in [0,1]$ and a row vector $v \in \R_{\geq 0}^{[0,k]}$ such that,
\begin{align}
  &\bullet ~\sum_{j' \in [0,k]}\mx_{i'j'} \in \Z_{\geq 0}\text{ for all } i' \in [1,i]
  ~~\bullet~~ \sum_{i'\in [\ell]}\mx_{i'j'} \in \Z_{\geq 0} \text{ for all }j' \in [0,k]  \\
  %& \bullet ~\sum_{i' \in [\ell], j'\in [k]} m_{j'} \log r_{i'} \mx_{i'j'} + \sum_{j' \in [k]}m_{j'} \log \rnew v_{j'}  \geq \sum_{i' \in [\ell], j'\in [k]} m_{j'} \log r_{i'} \my_{i'j'}\\
  & \bullet \sum_{i' \in [\ell]} r_{i'} \sum_{j'\in [0,k]}\mx_{i'j'} + \rnew \sum_{j' \in [0,k]} v_{j'}=\sum_{i' \in [\ell]} r_{i'} \sum_{j'\in [0,k]}\my_{i'j'} \\
& \bullet ~\sum_{j' \in [0,k]}v_{j'} \in \Z_{\geq 0}~~\bullet~ \sum_{i' \in [\ell]}\mx_{i'j'}+v_{j'}=\sum_{i' \in [\ell]}\my_{i'j'} \text{ for all }j' \in [0,k]\\
& \bullet ~\bg(\concat(\mx,v)) \geq \exp(-\log n) \bg(\my)~.
\end{align}
%Furthermore the running time the algorithm is $O()$. \zhihao{time complexity: we only need $O(\ell)$ time to describe the new matrix, but the assign operation on matrix is already $O(\ell\cdot k)$}
\end{lem}


==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}{}
  \item Did you describe the limitations of your work?
    \answerYes{See \Cref{sec:results}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> new_rounding.tex <==
\begin{lemma}
The optimizer $\mx^{*}$ of the optimization problem,
$$\max_{\mx \in \bZ}\bg(\mx)~,$$
is of the form $\mx^{*}_{ij}=x_i y_j r_i^{m_j}$, where $x_i$ and $y_j$ satisfy the following,
$$\sum_{j}$$
\end{lemma}
\begin{proof}
\begin{align}
    \mx_i=\sum_{j}\mx_{ij}=x_i\sum_{j}y_jr_i^{m_j}~.
\end{align}
Therefore $x_i=\frac{\mx_i}{\sum_{j}y_jr_i^{m_j}}~.$ Similarly we also have, $y_j=\frac{\phi_j}{\sum_{i}x_ir_{i}^{m_j}}~.$
Therefore for any $j$ and $j'$ such that $m_j \in [(1-\epsilon)m_{j'},(1+\epsilon)m_{j'}]$, we have that,
\begin{align}
    \mx_{ij} & =x_iy_jr_i^{m_j}  =x_i\frac{\phi_j}{\sum_{i'}x_{i'}r_{i'}^{m_j}} r_i^{m_j},\\
    &=x_i\frac{\phi_{j'}}{\sum_{i'}x_{i'}r_{i'}^{m_{j'}}} r_i^{m_{j'}} \cdot \frac{\phi_j}{\phi_{j'}} \cdot  \frac{\sum_{i'}x_{i'}r_{i'}^{m_{j'}}}{\sum_{i'}x_{i'} r_i^{m_j}} \frac{r_{i}^{m_j}}{r_i^{m_{j'}}},\\
    &=\mx_{ij'}\cdot \frac{\phi_j}{\phi_{j'}} \cdot  \frac{\sum_{i'}x_{i'}r_{i'}^{m_{j'}}}{\sum_{i'}x_{i'} r_i^{m_j}} \frac{r_{i}^{m_j}}{r_i^{m_{j'}}}~.
\end{align}
Therefore,
$$\frac{\mx_{ij}}{\phi_j} = \frac{\mx_{ij'}}{\phi_{j'}}\cdot  \frac{\sum_{i'}x_{i'}r_{i'}^{m_{j'}}}{\sum_{i'}x_{i'} r_i^{m_j}} \frac{r_{i}^{m_j}}{r_i^{m_{j'}}}~.$$
Consider the last term in the equation,
\begin{equation}
\frac{\sum_{i'}x_{i'}r_{i'}^{m_{j'}}}{\sum_{i'}x_{i'} r_{i'}^{m_j}} \cdot \frac{r_{i}^{m_j}}{r_i^{m_{j'}}} \leq  
\end{equation}
\begin{align}
    r_i^{m_j} \leq r_i^{(1+\epsilon)m_{j'}} \leq r_i^{m_{j'}} r_{i}^{\epsilon }
\end{align}
\end{proof}

\begin{algorithm}[H]
	\caption{Transfer$(\mx,i)$}\label{alg:round2}
	\begin{algorithmic}[1]
	\State Let $a_j=\sum_{j'=1}^{j-1}\mx_{i,j}$, $b_j=\sum_{i'=1}^{i-1}\mx_{i',j}$ and $c_j=\mx_{i,j}$ for all $j \in [k]$.
	\State Let $\my=\mx$.
		\For{$j=2\dots k-1$} 
		\State Let $\alpha=\min(a_{j},b_j)$.
		\State $\my_{i,j}=\my_{i,j}+\alpha~.$
		\State $\my_{i,j-1}=\my_{i,j-1}-\alpha~.$
		
		\EndFor
	\end{algorithmic}
	\label{alg:final}
\end{algorithm}

\begin{algorithm}[H]
	\caption{ApproximatePML$(\phi,\bR,\mx,i)$}\label{alg:round2}
	\begin{algorithmic}[1]
	\State Let $a_j=\sum_{j'=1}^{j-1}\mx_{i,j}$, $b_j=\sum_{i'=1}^{i-1}\mx_{i',j}$ and $c_j=\mx_{i,j}$ for all $j \in [k]$.
	\State Let $\my=\mx$.
		\For{$j=2\dots k-1$} 
		\State Let $\alpha=\min(a_{j},b_j)$.
		\State $\my_{i,j}=\my_{i,j}+\alpha~.$
		\State $\my_{i,j-1}=\my_{i,j-1}-\alpha~.$
		
		\EndFor
	\end{algorithmic}
	\label{alg:final}
\end{algorithm}

\begin{lemma}
Let $\mx \in \R_{\geq 0}^{\ell \times k}$ ($\ell << k$) such that, $\sum_{i' \in [\ell]}\mx_{i'j} \in \Z_{\geq 0} \text{ for all } j \in [k]$. Let $i \in [\ell]$ be an index such that,
$$\sum_{j \in [k]}\mx_{i'j} \in \Z_{\geq 0} \text{ for all } i' <i~.$$
Output a matrix $\my \in \R_{\geq 0}^{\ell \times k}$ and a index $j'$ such that $\|\my-\mx\|_1 \leq O(1)$ and,
$$\sum_{i \in [\ell], j\in [k]} m_j \log r_i \my_{ij} \geq \sum_{i \in [\ell], j\in [k]} m_j \log r_i \mx_{ij},~ \sum_{i \in [\ell]}\my_{ij}=\sum_{i \in [\ell]}\mx_{ij} \text{ for all } j \in [k],~ \sum_{j \in [k]}\my_{ij} =\sum_{j \in [k]}\mx_{ij} \text{ for all } i \in [\ell],$$
and 
$$\sum_{i'=1}^{i-1} \my_{i'j'} \in \Z_{\geq 0} \text{ and } \my_{ij'}-\lfloor \my_{ij'} \rfloor=\sum_{j \in [k]}\mx_{ij} - \lfloor \sum_{j \in [k]}\mx_{ij} \rfloor~.$$
where $m_j \in \Z_{\geq 0}$ and $r_i \in (0,1)$ $m_1>m_2>\dots >m_k$ and $r_1>r_2>\dots>r_\ell$.
\end{lemma}
\begin{proof}
We first introduce some notations, 
$$\beta_j \defeq \sum_{i' <i}\mx_{i'j},~~ \gamma_j = \mx_{ij},~~ \alpha_{1,j}=\sum_{j'<j}\mx_{ij'},~~ \text{ and }\alpha_{2,j}=\sum_{j'>j}\mx_{ij'}~.$$
\paragraph{Case 1} There exists an index $j$ such that, $\alpha_{1,j}=\beta_j$. In this case define $\my$ as follows,
$$\my_{i'j'}=\mx_{i'j'}$$




\begin{bmatrix}
	\vdots& \vdots &\vdots\\
	\hdots& \hdots &\hdots\\
	\vdots& \vdots &\vdots
\end{bmatrix}

\end{proof}

==> overview.tex <==
\kk{TODO}

==> proof_lem_final.tex <==
\section{Proof of \Cref{lem:final}}
\begin{proof} 
We first show that $\mxfinal \in \bZfinal$. Consider the matrix $\mxfinal=\my^{(\ell-1)}$, which by \Cref{lem:iteri} satisfies $\mxfinal \in \textbf{Z}^{\phi,frac}_{\bRfinal}$. Therefore to show that $\mxfinal \in \bZfinal$, all we need is a proof that $\mxfinal$ has integral row sums. By \Cref{lem:iteri}, we get that the matrix $\mx^{(\ell-1)}$ satisfies, $\sum_{j \in [k]}\mx^{(\ell-1)}_{ij} \in \Z_{\geq 0} \text{ for all } i \in [\ell-1]$ and $\sum_{i\in [\ell]}\sum_{j \in [k]}\mx^{(\ell-1)}_{ij} \in \Z_{\geq 0}$. Therefore, we have that, $\sum_{j \in [k]}\mximo_{\ell j} \in \Z_{\geq 0},$ which means that all the row sums of the matrix $\mx^{(\ell-1)}$ are integral.
Our final matrix $\mxfinal$ is a concatenation of $\mx^{(\ell-1)}$ and vectors $\vo,\dots \vl$, which by \Cref{lem:iteri} are known to have integral row sums. Therefore, the row sums of the matrix $\mxfinal$ are all integral and we conclude the proof for this case.

In the remainder of the proof, we show that $\bg(\mxfinal) \geq \exp(-O(\ell \log n)) \bg(\mx)$. Note that by \Cref{lem:iteri}, we have that,
$$\bg(\my^{(i)}) \geq \exp(-O(\log n)) \bg(\my^{(i-1)}) \text{ for all }i\in [\ell-1]~.$$
Furthermore, note that $\my^{(i)}=\my^{(i-1)}$, if $i-1$ corresponds to an integral row sum. By \Cref{lem:sparse}, we have that the number of non-zero rows is at most $\min(k,|\bR|)$ and we incur a loss of at most $\exp(-O(\log n))$ for each of these non-zero rows. Therefore our final matrix satisfies,
$$\bg(\my^{(\ell-1)}) \geq \exp(-O(\min(k,|\bR|) \log n)) \bg(\my^{(0)}) ~.$$
Equivalently,
$$\bg(\mxfinal) \geq \exp(-O(\min(k,|\bR|) \log n)) \bg(\mx) ~,$$
and we conclude the proof.
\end{proof}


==> proof_swap.tex <==
\begin{figure}[ht]\label{fig1}
\centering
\includegraphics[scale=0.3]{swap-crop.pdf}
\caption{Pictorial representation of $\swap$ operation.}
\end{figure}

==> rounding.tex <==
\begin{lemma}
	For any pseudo-distribution $\bq \in \psimplex$, profile $\phi \in \Phi^n$, let $\bq_1 \geq \bq_{2} \geq \dots \bq_{N}$ and $m_1 \geq m_{2} \geq \dots m_{N}$ be the probabilities and frequencies. For any $S\subset [N]$ we have,
	$$ \prod_{i \in S}\bp_{i}^{m_{i}} \prob{\bp_{\bar{S}},\phi_{\bar{S}}} \leq \prod_{x \in S} \prob{\bp,\phi} \leq \exp{ O(|S| \log N)} \prod_{i \in S}\bp_{i}^{m_{i}} \prob{\bp_{\bar{S}},\phi_{\bar{S}}}$$
	\end{lemma}
\begin{proof}
	\begin{align}
		\prob{\bp,\phi} &= cc_{\phi} \sum_{\sigma \in S_{[N]}} \prod_{x \in [N]}\bp_{x}^{m_{\sigma(x)}},\\
		&=\sum_{\{S'\subseteq [N]~|~|S'|=|S||\}}  \left(\sum_{\sigma_1 \in S_{S'}} \prod_{x \in S'}\bp_{x}^{m_{\sigma_1(x)}} \right) \left(\sum_{\sigma_2 \in S_{\bar{S'}}} \prod_{y \in \bar{S}}\bp_{y}^{m_{\sigma_2(y)}} \right),\\
		& \leq \binom{N}{|S|} \max_{\{S'\subseteq \bX~|~|S'|=|S||\}}  \left(\sum_{\sigma_1 \in S_{S'}} \prod_{x \in S'}\bp_{x}^{m_{\sigma_1(x)}} \right) \left(\sum_{\sigma_2 \in S_{\bar{S'}}} \prod_{y \in \bar{S}}\bp_{y}^{m_{\sigma_2(y)}} \right),\\
		& \leq \binom{N}{|S|} (|S|!) \max_{\{S'\subseteq \bX~|~|S'|=|S||\}}  \prod_{i \in S}\bp_{i}^{m_{i}} \left(\sum_{\sigma_2 \in S_{\bar{S'}}} \prod_{y \in \bar{S}}\bp_{y}^{m_{\sigma_2(y)}} \right),\\
	\end{align}
\end{proof}

\begin{lemma}[Bounds on the probability values]
Given $n$ i.i.d samples from a distribution $\bp$, for any $x \in \bX$ such that $\bp_{x} \geq \frac{1}{n^{1/3}}$,
$$\prob{n_{x}\leq \frac{1}{2} n^{2/3}} \leq \exp(-O(n^{2/3}))$$
\end{lemma}
\begin{proof}
 By chernoff bound,
 \begin{align}
     \prob{n_{x}\leq \frac{1}{2} n^{2/3}} &= \prob{n_{x}\leq (1-\delta) n^{2/3}} \leq \prob{n_{x}\leq (1-\delta) n \bp_{x}}\\ 
     & \leq  \exp(-\frac{n \bp_{x}}{12}) \leq \exp(-\frac{n^{2/3}}{12})~.
 \end{align}
\end{proof}



High level sketch of the algorithm:
\begin{enumerate}
	\item W.l.o.g we can assume that we know the approximate value of $c*$, which we call as $c'$ and assume that the given probability discretization set $\bR$ includes this scaling.
	\item The goal is to return a distribution such that,
	 $$\prob{\bpp,\phi} \geq \exp(-n^{1/3} \log n) \max_{\bS \in \bZ}\bg(\bS)~,$$
	 where $\bZ\subset \R_{\geq 0}^{\ell \times (k+1)}$ be the set of non-negative matrices, such that any $\bS \in \bZ$ satisfies,
	 \begin{equation}\label{eq:zrphi}
	 \sum_{i\in[1,\ell]}\bS_{i,j}=\phi_{j} \text { for all }j \in [1,k], \sum_{j\in[0,k]}\bS_{i,j} \in \Z \text { for all }i \in [1,\ell] \text{ and } \sum_{i \in [1,k]} \ri \sum_{j \in [0,k]}\bS_{i,j}\leq 1~.
	 \end{equation}
	 \item Define the following subsets of probability discretization set $\bR$. 
	 $$\bR_{1}\defeq \{\ri \in \bR~|~\ri \geq n^{-1/3}\} \text{ and }I_{1} \defeq \{i \in [1,\ell]~|~ \ri \in \bR_{1} \}~,$$
	 $$\bR_{2}\defeq \{\ri \in \bR~|~n^{-1/3}>\ri > n^{-2/3}\} \text{ and }I_{2} \defeq \{i \in [1,\ell]~|~ \ri \in \bR_{2} \}~,$$
	 $$\bR_{3}\defeq \{\ri \in \bR~|~\ri \leq n^{-2/3}\} \text{ and }I_{3} \defeq \{i \in [1,\ell]~|~ \ri \in \bR_{3} \}~.$$
	 \item Given $N_1,N_2,N_3$ and $x_1,x_2,x_3$ define the following optimization problem
	 
	 Consider the following optimization problem:
	 \begin{equation}
	 \max_{\bS \in \bZ}\bg(\bS)
	 \end{equation}
	 \begin{align*}
	 	\max_{x_{1},x_{2},x_{3} \in [0,1]} \max_{N_1,N_2,N_3 \in \Z} & \max_{\bS \in \bZ}\bg(\bS)\\
	 	\text{such that, }& \sum_{i \in I_{o}} (\bS \onevec)_{i}\ri = x_{o} \text{ for all }o \in \{1,2,3\}~, \\
	 	& \sum_{i \in I_{o}} (\bS \onevec)_{i} = N_{o} \text{ for all }o \in \{1,2,3\}~. \\
	 \end{align*}
	 \item We consider the following two cases separately: $N_2 < n^3$ and $N_2 \geq n^3$.
	 \item \text{Case 1}: $N_2 < n^3$ run $\mainalgone$.
	 \item \text{Case 2}: $N_2 \geq n^3$ run $\mainalgtwo$.
\end{enumerate}

Define two class of distributions $\Delta_1 = \{\bq \in \psimplex~|~ \sum_{x~|~\bq_{x} \geq n^{-2/3}}1 < n^{1/3} \}$ and $\Delta_2=\psimplex \backslash \Delta_1$.

Let $\bR_1 = \{\ri \in \bR~|~\ri \geq n^{-1/3} \}$, $\bR_2 = \{\ri \in \bR~|~n^{-1/3} \geq \ri \geq n^{-2/3} \}$ and $\bR_3= \{\ri \in \bR~|~\ri \leq n^{-2/3} \}$.
\begin{algorithm}[H]
	\caption{Algorithm for approximate PML distributions over $\Delta_1$}\label{mainalgone}
	\begin{algorithmic}[1]
		\Procedure{ProxyApproximatePML1}{$\phi,\bR$}
		\State {\bf Input}: Profile $\phi \in \Phi^n$ and probability discretization set $\bR$.
		\State {\bf Output}: A distribution $\bpapprox$.
		\State Perform empirical distribution on the top $n^{1/3}$ elements.
		\State Solve $\bSp=\argmax_{\bS\in \bZfrac} \log \bg(\bS)$. 
		\State Use \Cref{alg:rounding} to round the fractional solution $\bSp$ to integral solution $\bSext \in \bZext$.
		\State Construct discrete pseudo-distribution $\qext$ with respect to $\bSext$ (See \Cref{defn:distS}).
		%by assigning $(\bS \onevec)_{i}$ number of domain elements probability $\ri$ 
		\State \textbf{return} $\bpapprox\defeq \frac{\qext}{\|\qext\|_1}$.
		\EndProcedure
	\end{algorithmic}
\end{algorithm}




\begin{algorithm}[H]
	\caption{Algorithm for approximate PML}\label{mainalg}
	\begin{algorithmic}[1]
		\Procedure{Proxy Approximate PML}{$\phi,\bR$}
		\State {\bf Input}: Profile $\phi \in \Phi^n$ and probability discretization set $\bR$.
		\State {\bf Output}: A distribution $\bpapprox$.
		\State Solve $\bSp=\argmax_{\bS\in \bZfrac} \log \bg(\bS)$. 
		\State Use \Cref{alg:rounding} to round the fractional solution $\bSp$ to integral solution $\bSext \in \bZext$.
		\State Construct discrete pseudo-distribution $\qext$ with respect to $\bSext$ (See \Cref{defn:distS}).
		%by assigning $(\bS \onevec)_{i}$ number of domain elements probability $\ri$ 
		\State \textbf{return} $\bpapprox\defeq \frac{\qext}{\|\qext\|_1}$.
		\EndProcedure
	\end{algorithmic}
\end{algorithm}




For any scalar $c\geq 0$ let $\opt_{c}\defeq \max_{\bq \in \simplex_{c \bR}}\prob{\bq,\phi} $.
\begin{lemma} 
	For any scalars $a,b \geq 0$ that satisfy $a(1-\epsilon) \leq b \leq a(1+\epsilon)$ the following inequality holds:
	$$\exp(-\epsilon n ) \leq  \frac{\opt_{b}}{\opt_{a}} \leq \exp(\epsilon n )~.$$
\end{lemma}
\begin{proof}
	
\end{proof}

Recall 
\begin{equation}
\log \bg_{1}(\bS)\defeq \sum_{i \in [1,\ell]} \sum_{j \in [0,k]}\bSij\log \ri^{\mj} -\sum_{i \in [1,\ell]} \sum_{j \in [0,k]}\bSij\log \bSij +\sum_{i \in [1,\ell]}\Si \log \Si ~.
\end{equation}
Let $\hp \defeq \{i\in [1,\ell]~|~\ri \geq n^{-1/3} \}$ and $\hf \defeq \{j\in [0,k]~|~\mj \geq n^{-1/3} \}$ be the set of high probability and frequency elements respectively. Let $\lp \defeq [1,\ell] \backslash \hp$ and $\lf \defeq [0,k] \backslash \hf$ denote their complements.
\begin{equation}
\sum_{i\in[1,\ell]}\bS_{i,j}=\phi_{j} \text { for all }j \in [1,k] \text{ and } \sum_{i \in [1,k]} \ri \sum_{j \in [0,k]}\bS_{i,j}\leq 1~.
\end{equation}

\begin{equation}
\log \bg_{2}(\bS)\defeq \sum_{i \in [1,\ell]} \sum_{j \in [0,k]}\bSij\log \ri^{\mj} -\sum_{i \in \lp} \sum_{j \in \lf}\bSij\log \bSij +\sum_{i \in \lp}\Si \log \Si ~.
\end{equation}

\begin{lemma}
For any $\bS$, $|\log \frac{\bg_{1}(\bS)}{\bg_{2}(\bS)}| \leq n^{1/3} \log n~.$
\end{lemma}
\begin{proof}
	The proof follows because, for each $\sum_{i \in \hp} \Si \leq n^{1/3}$ and $\sum_{j \in \hf} \Sj \leq n^{1/3}$, therefore, 
	$$| -\sum_{i \in \hp} \sum_{j \in [0,k]} \bSij \log \bSij + \sum_{i \in \hp}\Si \log \Si| \leq n^{1/3} \log n~.$$
	$$| -\sum_{i \in [1,\ell]} \sum_{j \in \hf} \bSij \log \bSij | \leq n^{1/3} \log n~.$$
	Therefore the lemma follows. 
	\end{proof}


\begin{lemma}
	Given a solution $\bS$ that satisfies the following:
	\begin{enumerate}
		\item $\sum_{i \in \mp} \Si \in \Z$
		
		\end{enumerate}
	\end{lemma}


\begin{algorithm}[H]
	\caption{Algorithm for approximate PML}\label{euclid}
	\begin{algorithmic}[1]
		\Procedure{Approximate PML}{$\phi,\bR$}
		\State {\bf Input}: Profile $\phi \in \Phi^n$ and probability discretization set $\bR$.
		\State {\bf Output}: A distribution $\bpapprox$.
		\State Solve $\bSp=\argmax_{\bS\in \bZfrac} \log \bg(\bS)$. 
		\State Use \Cref{alg:rounding} to round the fractional solution $\bSp$ to integral solution $\bSext \in \bZext$.
		\State Construct discrete pseudo-distribution $\qext$ with respect to $\bSext$ (See \Cref{defn:distS}).
		%by assigning $(\bS \onevec)_{i}$ number of domain elements probability $\ri$ 
		\State \textbf{return} $\bpapprox\defeq \frac{\qext}{\|\qext\|_1}$.
		\EndProcedure
	\end{algorithmic}
	\label{alg:newfinal}
\end{algorithm}




\begin{lemma}
	For any distribution $\bp$ and $x \in \bX$, the frequency of element $x$ is a   
	\end{lemma}
\begin{proof}
	For any $x \in \bX$, the frequency of element $x$ is distributed $Bin(np(x))$. By the Chernoff bounds, we get that,
	\begin{equation}
	\prob{|f_{x} - n p(x)| \geq \frac{1}{2} np(x)} \leq \expo{-\frac{1}{12} n p(x)}~.
	\end{equation}
	
\end{proof}

\subsection{Case $r_{i} \leq n^{-1/3}$}

\begin{algorithm}[H]
	\caption{Rounding Algorithm}
	\begin{algorithmic}[1]
		\Procedure{Rounding}{$\bS$}
		\State {\bf Input}: Probability discretization set $\bR$, profile $\phi \in \Phi^{n}$ and $\bS \in \bZfrac \subseteq \R^{[1,\ell]\times \ztbtt}$.
		\State {\bf Output}: Probability discretization set $\bRext$ and $\bSext$.% \in \bZone$.
		\State {\bf Step 1}:
		\State Solve $\bRp \defeq \argmax_{\bRp} \log \bg(\bS,\bRp)~.$
		\State Let $\ma=$
		\State \textbf{return} $\bRext$ and $\bSext$.
		\EndProcedure
	\end{algorithmic}
	\label{alg:newrounding}
\end{algorithm} 



\begin{lemma}
	$$\bg(\bS,\bRp) \geq \bg(\bS,\bRp) \text{ and } \log \bg(\bS,\bRp)= n \cdot\sum_{i \in [1,\ell]}\Si \rip \log \rip -\sum_{i,j}\bSij \log \bSij \sum_{i \in [1,\ell]}\Si \log \Si~.$$
\end{lemma}

The solution $\bSp$ satisfies one of the following two conditions:
\begin{enumerate}
	\item $\sum_{\{i~|~ n^{-2/3}\leq \rip \leq n^{-1/3}\}} \Si \rip \geq n^{-1/3}~$.
	\item $\sum_{\{i~|~ n^{-2/3}\leq \rip \leq n^{-1/3}\}} \Si \rip < n^{-1/3}~$.
\end{enumerate}
\newcommand{\Spi}{(\bS'\onevec)_{i}}
\textbf{Case 1:}
\begin{enumerate}
	\item Note that $\sum_{\{i~|~ n^{-2/3}\leq \rip \leq n^{-1/3}\}} \Si \in \Z$.
	\item Let $x=\sum_{\{i~|~ n^{-2/3}\leq \rip \leq n^{-1/3}\}} \Si \rip$,\\
	 then 
	 \begin{align*}
	 \bg(\bS',\bRp)& =n \cdot\sum_{i \in [1,\ell]}\Spi \rip \log \rip + n \cdot\sum_{j}\sum_{i \in [1,\ell]}(S_{ij}-S'_{ij}) r_{i} \log (S_{ij}-S'_{ij}) r_{i} + \\
	 &=n \cdot\sum_{i \in [1,\ell]}\Si \ri p \log \rip + n \cdot\sum_{i \in [1,\ell]}\sum_{j}S_{ij} (1-c_{i})r_{i} \log S_{ij} (1-c_{i}) + \\
	 \end{align*}
	 
	 
	 
\end{enumerate}

\newcommand{\hpalg}{\mathrm{HighProbabilityRound}}

\begin{lemma}
	Given a profile $\phi$, probability mass value $x$, cardinality parameter $N$ and probability discretization set $\bR$. The algorithm $\hpalg(\phi,\bR)$ returns a solution pair $(\bSp,\bRp)$ that satisfies:
	\begin{itemize}
		\item $\bSp \in \Z^{\ell' \times k}$ for some non-negative integer $\ell' =|\bRp|$.
		\item $\bg(\bSp,\bRp) \geq \exp(-N \log N) \max_{\bS \in \textbf{Z}_{\bR,x,N}} \bg(\bS,\bR)~.$
	\end{itemize}
	\end{lemma}
\begin{proof}
	$$\sum_{i \in [1,\ell]} \sum_{j \in [0,k]}\bSp_{ij}\log \rip^{\mj} \geq \max_{}~.$$
\end{proof}

\newcommand{\mpalg}{\mathrm{MidProbabilityRound}}

\begin{lemma}
	Given a profile $\phi$
	\end{lemma}

\newcommand{\lpalg}{\mathrm{LowProbabilityRound}}
\begin{lemma}
	Given a profile $\phi$, probability discretization set $\bR$ such that each $\ri \in \bR$ satisfies $\ri \leq \gamma$ and a solution $\bS \in \bZfrac$. The algorithm $\lpalg(\phi,\bR,\bS)$ returns a solution pair $(\bSp,\bRp)$ such that:
	$$\bg(\bSp,\bRp) \geq \exp(-\gamma n \log n) \bg(\bSp,\bRp)~.$$
	\end{lemma}
\begin{proof}
 Refer our distinct approx paper.
\end{proof}

==> structure.tex <==

\newcommand{\mxstar}{\mx^{*}}

Consider the following optimization problem:
\begin{equation}\label{eq:convopt}
    \max_{\mx \in \bZfrac} \log \bg(\mx)
\end{equation}
Explicitly writing the objective and the constraint set gives us:
\begin{align*}
    \max_{\mx \in \R_{\geq 0}^{[1,\ell]\times [0,k]}}& \sum_{i\in[1,\ell],j\in[0,k]}\left[(\mj \log \ri)\mx_{ij} -\mx_{ij}\log\mx_{ij}\right]+\sum_{i\in[1,\ell]}[\mx\vones]_{i}\log[\mx\vones]_{i}\\
    &\text{such that }~ [\mx^\top \cones]_{j}=\phi_{j} \text { for all }j \in [1,k] \text{ and } \vr^{\top} \mx \rones\leq 1~.
\end{align*}

Assume $m_j < m_{j+1}$ and $r_{i} < r_{i+1}$.

\begin{lemma}
Let $\mxstar$ be the optimal solution to optimization problem \ref{eq:convopt}, then $\mxstar$ satisfies for all $i\in [1,\ell-1]$ and $j \in [0,k]$:
$$\frac{1}{\|\mxstar_i\|_1}\sum_{a \in [0,j]} \mxstar_{i,a} \geq \frac{1}{\|\mxstar_{i+1}\|_1}\sum_{a \in [0,j]} \mxstar_{i+1,a}~.$$
Equivalently,
$$\frac{1}{\|\mxstar_i\|_1}\sum_{a \in [j,k]} \mxstar_{i,a} \leq \frac{1}{\|\mxstar_{i+1}\|_1}\sum_{a \in [j,k]} \mxstar_{i+1,a}~.$$
\end{lemma}

\begin{proof}

Given a distribution $p$ such that $p_1>p_2>\dots > p_k$ and frequencies $n_1>n_2>\dots n_k$.

Let $P_{ij}$ denotes the conditional probability of $p_i$ generating frequency $n_j$.

We want to show that,
$$\sum_{j\leq k}P_{1,j} \geq \sum_{j\leq k}P_{2,j}$$

Conditional probability of generating top $k$ frequency elements for $p_1$.
$$\sum_{i=1}^{k}\sum_{j\neq i} p_1^{n_i} p_2^{n_j} c_{ij}~.$$
Conditional probability of generating top $k$ frequency elements for $p_2$.
$$\sum_{i=1}^{k}\sum_{j\neq i} p_2^{n_i} p_1^{n_j} c_{ij}~.$$

Note that $c_{ij}=c_{ji}$. In the remainder we prove the lemma term by term.

Consider any $i \in [1,k]$ and $j \neq i$, we divide the analysis into two cases:
\begin{itemize}
    \item If $j \in [1,k]$, as $c_{ij}=c_{ji}$ we note that the coefficient of terms with $c_{ij}$ is $p_1^{n_i} p_2^{n_j} + p_1^{n_j} p_2^{n_i}$ in both the conditional probabilities.
    
    \item If $j>k$, then we note that the coefficient of $c_{ij}$ in the first and second conditional probabilities corresponding to $p_1$ and $p_2$ are $p_1^{n_i} p_2^{n_j}$ and $p_2^{n_i} p_i^{n_j}$ respectively. As $n_i>n_j$ (because $j>k$) we get the desired result.
\end{itemize}

\end{proof}
